NeurMiPs: Neural Mixture of Planar Experts for View Synthesis

We present Neural Mixtures of Planar Experts (NeurMiPs), a novel planar-based scene representation for modeling geometry and appearance. NeurMiPs leverages a collection of local planar experts in 3D space as the scene representation. Each planar expert consists of the parameters of the local rectangular shape representing geometry and a neural radiance field modeling the color and opacity. We render novel views by calculating ray-plane intersections and composite output colors and densities at intersected points to the image. NeurMiPs blends the efficiency of explicit mesh rendering and flexibility of the neural radiance field. Experiments demonstrate superior performance and speed of our proposed method, compared to other 3D representations in novel view synthesis.

==> figures/1_teaser.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-5mm}
    \includegraphics[width=.95\linewidth]{figures/images/teaser.png}
\vspace{-5mm}
   \caption{\textbf{A Comparison of Different 3D Representations for Neural Rendering.} \emph{Neural implicit surface} models accurate surface geometry but rendering requires expensive sequential sampling. 
   \emph{Multi-planar imagery} is efficient, but does not reflect true geometry
   and is not suitable for extrapolation. While 
   NeRF is flexible, it is not sample-efficient and its learned density field might not reflect true scene geometry. Our proposed \emph{Mixture of Planar Experts} is efficient and is able to model complicated surface geometry and appearance.
}
    \label{fig:comparison}
\vspace{-5mm}
\end{figure*}

==> figures/3_bake_filter.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/images/Blank_image.jpg}
    \caption{\textbf{Illustration of rendering acceleration.} After training, we bake view-independent transparency $\alpha$ on each planes, and ignore ray-plane intersections with small weights for alpha composite, which enhance rendering efficiency significantly. Note that the point clouds are normalized into a zero-mean unit sphere.}
    \label{fig:3_bake_filter}
\end{figure}

==> figures/3_fit_planes.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/images/rmse_point2rec.jpg}
    \caption{\textbf{RMSE between points and rectangles.} We fit several learnable planes on point clouds of two different scenes. With plane number increasing, the RMSE between point and bounded planes (rectangles) can be reduced significantly, which indicates that planes are able to approximate complex real-world geometry.}
    \label{fig:3_fit_planes}
\end{figure}

==> figures/4_depth.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/images/cumulative_depth.png}
    \caption{\textbf{Cumulative Depth Error.} $(x, y)$ indicates that there are $y\%$ pixels with absolute error lower than $x$.}
    \vspace{-3mm}
    \label{fig:4_depth}
\end{figure}

==> tables/4_depth_metrics.tex <==
\begin{table}[]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
        \hline 
        Model & MAE $\downarrow$ & Median $\downarrow$ & \makecell{Outlier (\%)\\ $\tau=0.2$} & \makecell{Outlier (\%)\\ $\tau=0.3$} & \makecell{Outlier (\%)\\ $\tau=0.4$}\\
        \hline
        NeX~\cite{Wizadwongsa2021NeX}      & 0.929 & 0.767 & 86.7 & 79.9 & 73.2\\
        NeRF~\cite{mildenhall2020nerf}     & \textbf{0.263} & 0.137 & 35.9 & 22.9 & \textbf{16.2}\\
        KiloNeRF~\cite{reiser2021kilonerf} & 0.364 & 0.125 & 40.8 & 32.8 & 27.1\\
        \hline
        Ours                               & 0.561 & \textbf{0.066} & \textbf{28.0} & \textbf{21.9} & 18.3\\
         \hline
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{\textbf{Depth estimation metrics.} MAE: Mean Absolute Error. Median: Median Error. Outlier: ratio of pixels with absolute error over threshold $\tau$.}
    \label{tab:4_depth_metrics}
\end{table}

==> tables/4_quantity_blendedmvs.tex <==
\begin{table}[h]
\centering
{
\scriptsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l|c|c|c}
 \hline
 Model & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$\\
 \hline 
 \hline 
 NeRF~\cite{mildenhall2020nerf}          & 27.29 & 0.91 & 0.07 \\ 
 NSVF~\cite{liu2020neural}               & 27.90 & 0.90 & 0.11 \\
 KiloNeRF~\cite{reiser2021kilonerf}      & 27.39 & 0.92 & 0.06 \\ 
 \hline
 Ours            & 26.27 & 0.88 & 0.098  \\
 \hline
\end{tabular}
}
\caption{\textbf{Quantitative results on BlendedMVS.} \shenlong{we mentioned additional results see supp and make it to train better with distillation}}
\label{tab:qantity_blendedmvs}
}
\end{table}

==> tables/4_quantity_replica.tex <==
\begin{table}[t]
\centering
\small
% \resizebox{\columnwidth}{!}
{
\begin{tabular}{ l|c|c|c|c|c } 
 \hline
 Model & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FPS$\uparrow$ & TFLOPs$\downarrow$\\
 \hline 
 \hline 
 NeRF~\cite{mildenhall2020nerf}  & 28.886 & 0.933 & 0.166 & 0.186 & 39.997\\ 
 NeX~\cite{Wizadwongsa2021NeX}   & 23.222 & 0.878 & 0.214 & 0.142 & 63.907\\
Ours & \textbf{29.780} & \textbf{0.936} & \textbf{0.144} & \textbf{2.13} & \textbf{0.681}\\
 \hline
\end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Quantitative Comparison on Replica.} 
}
\label{tab:4_quantity_replica}
\vspace{-5mm}
\end{table}

==> tables/4_quantity_replica_difficulty.tex <==
\begin{table*}[t]
\vspace{-5mm}
%\resizebox{\textwidth}{!}
\begin{center}
\small
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\hline 
    & \multicolumn{3}{c}{Easy} & \multicolumn{3}{c}{Medium}  & \multicolumn{3}{c}{Hard} \\
    & PSNR $\uparrow$    & SSIM $\uparrow$   & LPIPS $\downarrow$   & PSNR $\uparrow$  & SSIM $\uparrow$ & LPIPS $\downarrow$   & PSNR $\uparrow$  & SSIM $\uparrow$      & LPIPS $\downarrow$   \\
\hline 
NeX~\cite{Wizadwongsa2021NeX}      & 25.88 & 0.844 & 0.136 & 24.56 & 0.828 & 0.156 & 23.86 & 0.826 & 0.164\\ 
NeRF~\cite{mildenhall2020nerf}     & 31.41 & \textbf{0.915} & 0.081 & 29.98 & \textbf{0.901} & 0.097 & 29.02 & 0.887 & 0.113 \\
PlenOctree~\cite{yu2021plenoctrees}& 28.05 & 0.877 & 0.171 & 27.613 & 0.872 & 0.174 & 27.51 & 0.866 & 0.179\\
KiloNeRF~\cite{reiser2021kilonerf} & 28.00 & 0.908 & 0.085 & 28.06 & 0.893 & 0.105 & 27.50 & 0.886 & 0.117 \\
\hline
Ours   & \textbf{31.98}  & 0.914  & \textbf{0.074} & \textbf{30.31} & 0.894 & \textbf{0.092} & \textbf{30.05} & \textbf{0.892} & \textbf{0.096} \\ 
\hline 
\end{tabular}
}
\vspace{-3mm}
\caption{\textbf{Quantitative Performance on Replica at Different Difficulty Levels.} 
}
\vspace{-3mm}
\label{tab:4_quantity_replica_difficulty}
\end{center}
\vspace{-5mm}
\end{table*}

==> tables/4_quantity_tanks_2.tex <==
\begin{table}[t]
\centering
\small

\scalebox{0.9}
{
\begin{tabular}{ l|c|c|c|c|c} 
 \hline
 Model & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & FPS & \#Params (M) \\
 \hline 
 NeRF            & 28.32 & 0.904 & 0.168 & 0.014 & 1.19\\
 KiloNeRF        & 28.41 & 0.910 & 0.090 & 12.73 & 6.21\\
 PlenOctrees$^1$  & 27.99 & \textbf{0.917} & 0.131 & - & -\\
 PlenOctrees$^2$  & 24.22 & 0.857 & 0.172 & 82.62 & 337.33\\
 \hline
 Ours         & \textbf{28.46} & 0.908 & \textbf{0.089} & 10.01 & 6.21\\
 \hline
\end{tabular}
}
\vspace{-3mm}
\caption{\textbf{Quantitative comparison on Tanks~\&~Temples.} PlenOctrees$^1$: reported in paper. PlenOctrees$^2$: reproduced with provided pretrained NeRF-sh.}
\label{tab:4_quantity_tanks}
\vspace{-1mm}

\end{table}
